ZeroRAG: Adaptive Semantic Peer Routing for Decentralized Retrieval-Augmented Generation

Retrieval-augmented generation (RAG) is a standard approach to enhance the reliability of large language model (LLM) outputs by retrieving documents relevant to a query and supplying them in the LLM prompt. Today's RAG systems collect, index, and serve these documents from centralized stores. In practice, however, documents are owned by organizations, devices, and individuals who cannot or will not surrender custody of them to a central party, e.g., because of privacy, copyright or regulatory compliance. Existing modern decentralized retrieval techniques either reintroduce a coordinating authority, or rely on a global data structure that requires continuous network-wide coordination (e.g., DHTs). We present ZeroRAG, a decentralized routing layer for document retrieval in RAG that performs semantic query routing across an overlay of peers with- out global data structures or centralized orchestration. Documents remain with the peers that own them, and each peer keeps only lightweight local state: a bounded set of neighbor advertisements and a cache of recently routed queries. Using these, ZeroRAG steers each query through a best-first walk that progressively rewires the overlay toward semantically relevant neighbors, so recall improves over time as the network self-organizes. We evaluate ZeroRAG using three real-world workloads and two decentralized baselines. We find that ZeroRAG outperforms baselines in terms of recall and required network messages, approaches the recall and LLM answer accuracy of a centralized document store, self-heals after catastrophic peer failures, and scales to 100 000 peers.

==> plots/amazon-retrieval-pct-rolling1000/amazon-retrieval-pct-rolling1000.tex <==
\noindent\begin{tikzpicture}
  \begin{axis}[
    xlabel={Rolling window (1k queries)},
    ylabel={Relevant retrieved (\%)},
    ymin=0, ymax=100,
    xmin=0,
    width=260.4pt,
    legend columns=2,
    legend style={font=\sffamily\scriptsize},
    % Cycle list (Dark2 colors x dashes x marks) is set globally in
    % plots/pgfstyle.tex; per-series color/dash/mark assignments are
    % left to it. Marks suppressed because 1k-window curves have too
    % many points for marker glyphs to be legible.
    every axis plot/.append style={thick, no marks, each nth point=4},
  ]
    % ZeroRAG family: blue, pinned via the `sys*` styles in
    % plots/pgfstyle.tex. All non-ZeroRAG series use plain `\addplot+`
    % so the Dark2 cycle picks color/dash/mark per-series.
    \addplot+[sys] table[col sep=comma, x=window_index, y={ZeroRAG}]
      {csv-files/amazon_retrieval_pct_rolling1000.csv};
    \addlegendentry{\sys}
    \addplot+[sys-dashed] table[col sep=comma, x=window_index, y={ZeroRAG no query memory}]
      {csv-files/amazon_retrieval_pct_rolling1000.csv};
    \addlegendentry{\sys (no query memory)}
    \addplot+[sys-dotted] table[col sep=comma, x=window_index, y={ZeroRAG no new connections}]
      {csv-files/amazon_retrieval_pct_rolling1000.csv};
    \addlegendentry{\sys (static topology)}
    \addplot+[sys-dashdot] table[col sep=comma, x=window_index, y={ZeroRAG no query memory and no new connections}]
      {csv-files/amazon_retrieval_pct_rolling1000.csv};
    \addlegendentry{\sys (no mem, static)}
    \addplot+ table[col sep=comma, x=window_index, y={Semantica}]
      {csv-files/amazon_retrieval_pct_rolling1000.csv};
    \addlegendentry{Semantica}
    \addplot+ table[col sep=comma, x=window_index, y={LSH w=0.75 k=10 L=20}]
      {csv-files/amazon_retrieval_pct_rolling1000.csv};
    \addlegendentry{LSH $w{=}0.75,k{=}10,L{=}20$}
    \addplot+ table[col sep=comma, x=window_index, y={LSH w=2.0 k=10 L=50}]
      {csv-files/amazon_retrieval_pct_rolling1000.csv};
    \addlegendentry{LSH $w{=}2.0,k{=}10,L{=}50$}
    \addplot+ table[col sep=comma, x=window_index, y={LSH w=2.5 k=10 L=50}]
      {csv-files/amazon_retrieval_pct_rolling1000.csv};
    \addlegendentry{LSH $w{=}2.5,k{=}10,L{=}50$}
    \addplot+ table[col sep=comma, x=window_index, y={LSH w=3.0 k=10 L=10}]
      {csv-files/amazon_retrieval_pct_rolling1000.csv};
    \addlegendentry{LSH $w{=}3.0,k{=}10,L{=}10$}
    \addplot+ table[col sep=comma, x=window_index, y={LSH w=3.0 k=10 L=20}]
      {csv-files/amazon_retrieval_pct_rolling1000.csv};
    \addlegendentry{LSH $w{=}3.0,k{=}10,L{=}20$}
    \addplot+ table[col sep=comma, x=window_index, y={LSH w=3.0 k=10 L=50}]
      {csv-files/amazon_retrieval_pct_rolling1000.csv};
    \addlegendentry{LSH $w{=}3.0,k{=}10,L{=}50$}
    \addplot+ table[col sep=comma, x=window_index, y={LSH w=3.0 k=8 L=50}]
      {csv-files/amazon_retrieval_pct_rolling1000.csv};
    \addlegendentry{LSH $w{=}3.0,k{=}8,L{=}50$}
    \addplot+ table[col sep=comma, x=window_index, y={LSH w=4.0 k=10 L=50}]
      {csv-files/amazon_retrieval_pct_rolling1000.csv};
    \addlegendentry{LSH $w{=}4.0,k{=}10,L{=}50$}
  \end{axis}
\end{tikzpicture}


==> sections/introduction_prism.tex <==
\section{Introduction (OpenAI Prism)}
\chatgpt{Entire section is AI-generated}

Machine learning is rapidly moving from centralized platforms into local, user-facing systems. Retrieval-augmented generation pipelines, personal assistants, edge analytics, and domain-specific copilots increasingly operate over data that is private, heterogeneous, dynamic, and distributed across devices or organizations. These applications require middleware that can connect models to useful context without assuming that all data can be collected, labeled, normalized, and maintained in a single managed repository. The traditional middleware stack was not designed for this setting: it often depends on centralized indexing, carefully curated schemas, supervised labels, or high-dimensional data structures whose performance and maintainability degrade as data grows richer and less predictable.

\textbf{Decentralized middleware}. This paper argues that emerging AI and machine learning systems need a different kind of middleware: decentralized, label-free, and robust to unstructured data. Decentralization is essential because many local ML applications must operate where data already resides, whether for privacy, latency, ownership, or regulatory reasons. Requiring data to be copied into a central service introduces trust and governance barriers, increases synchronization costs, and limits deployment in personal, institutional, and edge environments. A decentralized middleware layer instead allows independently managed data sources, models, and agents to participate in computation while preserving local control.

Equally important, such middleware should not depend on data labeling as a prerequisite for use. Labeling is expensive, slow, domain-specific, and often infeasible for the long tail of local application data: notes, documents, logs, code repositories, messages, experimental records, and multimodal artifacts. Systems such as local RAG pipelines need to become useful immediately over existing collections, then improve as users interact with them. Middleware for this setting should therefore support discovery, retrieval, routing, and adaptation from weak signals, self-supervised representations, metadata, feedback, and runtime behavior rather than from large manually labeled datasets.

Finally, middleware must avoid brittle data-structure upkeep that collapses under the curse of dimensionality. Modern ML data is represented through embeddings, latent features, graphs, traces, and multimodal context, all of which evolve as models, documents, and user goals change. Maintaining rigid indexes, schemas, or handcrafted feature structures can become a dominant operational cost, while nearest-neighbor structures and similarity metrics may degrade as dimensionality, heterogeneity, and distribution shift increase. A practical middleware layer must therefore be adaptive: able to organize, query, and refresh representations incrementally without assuming stable schemas or requiring constant manual reengineering.

\textbf{Middleware as infrastructure}. The central challenge is to provide the coordination benefits of middleware without imposing the centralization and curation assumptions of earlier systems. We frame middleware for local AI and machine learning applications as an infrastructure layer that mediates among data sources, representation models, retrieval mechanisms, and application agents. Its role is not merely to move data, but to make decentralized and weakly structured information actionable for models at runtime. By focusing on decentralized operation, label-free learning signals, and low-upkeep representation management, this track can address the infrastructure gap between powerful foundation models and the messy, private, evolving data environments in which they are increasingly deployed.

\textbf{Decentralized RAG}. We define a RAG as a ...
\TODO{Define}.


% \section{RAG storyline introduction}
% \begin{enumerate}
%     \item [Quinten] We want a solution that is decentralized, does not require data labeling, and does not require data structure upkeep (or collapse due to the curse of dimensionality). Application: local RAG.


%     \item We propose a method to organise p2p networks into semantically relevant neighbourhoods, beating previous works on the same topic, all the while ensuring that the incentives align to allow users to participate while not holding data they're not interested in. The goal is to maximize distributed target recall under a bounded peer-contact budget, while avoiding a global index, centralized coordinator, or a global data structure.  The routing problem is therefore constrained: each peer may use only its local documents, outgoing neighbor state, and previously observed routed-query memory.
% \end{enumerate}

% \section{RAG Storyline 2}
% \begin{itemize}
%     \item RAG retrieval is usually centralized: most systems assume a central vector database in the form of either a server or a federated system, which is censorship prone, central failure prone and less scalable than when documents are distributed across many peers.

%     \item In a peer-to-peer setting, the real problem is decentralized semantic routing: a peer cannot search a global index and must choose which peers to contact using only local documents, neighbor state, advertisements, and routed-query memory.

%     \item Global structures are a poor fit for this setting: DHTs, semantic tries, centroids, and blockchain-style shared state still require maintained structure under churn, document updates, and changing peer interests.

%     \item \textsc{ZeroRAG} makes the overlay itself the retrieval structure: peers route queries through semantically promising neighbors and update their connections based on successful or high-scoring routes.

%     \item Over time, query traffic causes the network to self-organize into useful semantic neighborhoods without labels, topic taxonomies, a central coordinator, or a globally maintained index.

%     \item The evaluation question is recall under bounded coordination: how much retrieval quality can be recovered when each query can contact only a limited number of peers.

%     \item Main thesis: \textsc{ZeroRAG} reframes RAG retrieval as a local peer-routing problem, where useful semantic neighborhoods emerge from query traffic instead of being imposed by a global index.
% \end{itemize}

==> sections/system_model.tex <==
\section{System model (Prism AI generated)}
\label{sec:system-model}

\chatgpt{Entire section is AI-generated}

We model a local retrieval-augmented machine learning system as a decentralized network of peers. Each peer represents an independently managed user, device, organization, or local agent that owns a private document inventory and issues queries over time. A peer may store notes, clicked documents, product records, logs, code, or other artifacts, but the middleware only assumes that these artifacts can be represented by embeddings and compared to query embeddings at runtime. Peers are connected by an overlay graph. A query begins at the issuing peer and is routed through this graph for a bounded number of rounds or peer contacts. Each contacted peer evaluates the query against its local inventory, returns matching documents or relevance evidence, and may provide routing information that helps the query reach other useful peers.

The main actors are \emph{queriers}, \emph{candidate peers}, \emph{routing state}, and \emph{reference infrastructure}. The querier is the peer that initiates a request and defines the information need. Candidate peers are remote peers contacted during routing; they contribute local vector comparisons, retrieved documents, and feedback about whether their inventories were useful. Routing state includes the current overlay neighborhood, any routed-query memory retained by peers, and any adaptive links created after successful retrievals. Reference infrastructure includes centralized baselines such as HNSW and structured decentralized baselines such as E2LSH-DHT; these are not required by \textsc{ZeroRAG}, but they provide comparison points for recall and vector-comparison cost.

Our first assumption is that data ownership is decentralized. Documents remain with the peers that hold them, and retrieval must work without collecting every document into a single managed service. This assumption matches the privacy, latency, ownership, and governance constraints that motivate local AI applications. The simulator therefore excludes the querier's own inventory when measuring distributed retrieval: success requires finding useful information at another peer rather than trivially reading a document already held locally. In experiments with seeded inventories, such as AOL-IA, this choice isolates the routing problem by asking whether the network can discover a relevant remote holder of the target document.

Our second assumption is that the system is label-free at deployment time. Peers need not provide manually curated classes, schemas, ontologies, or supervised training labels before participating in the network. Instead, the middleware relies on weak operational signals: query embeddings, document embeddings, local similarity comparisons, clicked or relevant documents in evaluation traces, repeated demand patterns, peer-specific topic preferences, and feedback from successful or failed routes. In Amazon Electronics, relevance is multi-valued because a category-derived query may correspond to many products for the same reviewer. In AOL-IA and the synthetic benchmark, the primary task is top-$1$ retrieval of a clicked or nearest-neighbor target. These settings differ in their relevance definitions, but all evaluate whether routing can exploit behavior and representation similarity without requiring a global labeling process.

Our third assumption is that representations and peer interests are heterogeneous but comparable. Documents and queries may originate from different users, categories, or topics, yet the system assumes they can be embedded into a shared vector space in which approximate semantic similarity is meaningful. The synthetic benchmark makes this assumption explicit by generating documents and queries around topic centroids on the unit sphere. The real-data experiments inherit the assumption from the embedding model used to encode queries and documents. We do not assume that embeddings are perfect, stable, or globally calibrated; rather, the middleware must tolerate noisy similarity estimates, repeated queries, uneven peer activity, and changing local inventories.

Our fourth assumption is that peers have bounded local and communication resources. A query cannot contact every peer, and a peer cannot necessarily store an unbounded history of documents or routed queries. The experimental knobs therefore include routing rounds, fanout, initial graph degree, routed-query memory size, FIFO local-capacity limits, document-inventory size, and user-population size. These limits define the practical operating regime of the system: recall must be achieved through selective routing and adaptive topology formation rather than exhaustive broadcast or centralized scanning.

The primary threats considered in this paper are operational rather than adversarial. The system may fail because the overlay graph is poorly connected, because useful peers are several hops away, because local inventories are sparse, because peer interests are highly skewed, because routed-query memory is too small, because document collections grow, or because peers churn. The ablations stress these threats directly by varying churn, document scale, FIFO capacity, fanout, graph degree, memory limits, and user-population size. We also treat high-dimensional representation cost as a threat: even when a centralized index can achieve high recall, the cost of maintaining and querying global high-dimensional structures may be undesirable for local, privacy-preserving systems.

We do not model Byzantine peers, poisoning attacks, malicious query rewriting, collusion, access-control enforcement, cryptographic privacy, or leakage from returned documents and embeddings. Peers are assumed to follow the protocol, return truthful local retrieval results, and maintain whatever local data they are allowed to expose to the middleware. This non-adversarial model is appropriate for the experiments in this paper because the goal is to measure whether decentralized, label-free routing can approach centralized retrieval quality under realistic resource and heterogeneity constraints. Security, privacy hardening, incentive compatibility, and adversarial robustness are important extensions, but they are outside the scope of the present evaluation.
